Graph-Based Shape Analysis Beyond Context-Freeness

We develop a shape analysis for reasoning about relational properties of data structures. Both the concrete and the abstract domain are represented by hypergraphs. The analysis is parameterized by user-supplied indexed graph grammars to guide concretization and abstraction. This novel extension of context-free graph grammars is powerful enough to model complex data structures such as balanced binary trees with parent pointers, while preserving most desirable properties of context-free graph grammars. One strength of our analysis is that no artifacts apart from grammars are required from the user; it thus offers a high degree of automation. We implemented our analysis and successfully applied it to various programs manipulating AVL trees, (doubly-linked) lists, and combinations of both.

==> Makefile <==
.PHONY: default clean distclean


default: main.pdf


main.pdf: *.tex bibliography.bib 
	pdflatex main

all:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

spellcheck:
	for f in *.tex; do aspell check $$f; done
	



clean:
	rm -f *.aux *.log *.bbl *.blg *~ main.pdf *.out *.synctex.gz *.backup

distclean: clean
	rm -f main.pdf


==> abstract.tex <==
Our abstract domain extends heap configurations by three aspects:

First, we introduce hyperedges that represent abstract parts of the heap, i.e. sets of graphs, such as all binary trees of arbitrary height.
Due to their similarity to summary nodes~\cite{chase1990analysis,Ferrara2015automatic,sagiv1996solving}, we will call them \emph{summary edges}.

The formal semantics of summary edges is defined in terms of \emph{hyperedge replacement grammars} (HRG) --- a well-established formalism for context-free graph rewriting~\cite{habel1992hyperedge}.
As the name suggests, this involves replacing hyperedges by graphs. 
Thus, as a second component, hypergraphs are extended by a sequence of \emph{external nodes} that specify how graphs are glued together during replacement.
Intuitively, our analysis then uses HRG derivations for concretization and inverse HRG derivations for abstraction.

HRGs are, however, not expressive enough to capture balanced data structures.
Hence, we lift the more powerful concept of \emph{indexed grammars} -- a classical extension of CFGs due to Aho~\cite{aho1968indexed} --- to graph grammars.
This leads to the third extension: 
We allow summary edges to be additionally labeled with an \emph{index}, i.e. a finite sequence of symbols.
Prefixes of these indices can then be accessed by the rules of a grammar to gain additional control over possible derivations.
For example, we use indices to model the set of all \emph{balanced} binary trees.


Before we discuss our analysis in detail, we extend heap configurations as described above.
Furthermore, we introduce indexed hyperedge replacement grammars as a device to guide abstraction and concretization.


\subsection{Indexed Heap Configurations} \label{sec:ihc}

We first formalize the previously discussed extensions of hypergraphs.

\begin{definition}%[Indexed Hypergraph]
\label{def:indexed-hg}
Let $S$ be a set equipped with a ranking function $\Rank : S \to \Nats$.
   Moreover, let $\I$ be a finite set of \emph{indices}.
   An \emph{indexed hypergraph} over $S$ and $\I$ is a tuple
   $\iH = (\V,\E,\Lab,\Att,\Ind,\Ext)$, where
   \begin{itemize}
     \item $(\V,\E,\Lab,\Att)$ is a hypergraph over $S$ according to Definition~\ref{def:hypergraph}, 
     \item $\Ind : E \to \I^{*}$ assigns an index sequence to each edge in $\E$, and
     \item $\Ext \in \V^{*}$ is a (possibly empty) repetition-free sequence of \emph{external nodes}.
   \end{itemize}
   %The set of all indexed hypergraphs over $S$ and $\I$ is $\IGraphs{S}{\I}$.
\end{definition}

As the focus of this paper lies on applying indexed hypergraphs as an abstract domain for shape analysis, we often assume the set of edge labels to consist of labels for variables, fields and summary edges.
More formally, let $\Sum$ be a set of \emph{summary symbols} that is disjoint from the set of variables $\Var$ and the set of fields $\Fields$. 
Since these three sets determine the possible type of an edge in our model, we set $\Types = \Var \cup \Fields \cup \Sum$.
Moreover, we fix some non-empty finite set $\Index$ of indices that includes a dedicated end-of-index symbol $\iBot$.
We next lift the concept of heap configurations to indexed hypergraphs.

\begin{definition}%[Indexed Heap Configuration]
\label{def:indexed-hc}
  An indexed hypergraph $\iH = (\V,\E,\Lab,\Att,\Ind,\Ext)$ over $\Types$ and $\Index$ is 
  an \emph{indexed heap configuration} if 
  \begin{itemize}
    \item its underlying hypergraph $(\V,\E,\Lab,\Att)$ is a heap configuration, 
    \item the unique $\Null$ node coincides with the first external node, i.e. $\vNull = \Elem{\Ext}{1}$, and
    \item the first node attached to each summary edge is $\vNull$, i.e. for each $e \in \E$ with $\Lab(e) \in \Sum$, we have $\Elem{\Att(e)}{1} = \vNull$.
  \end{itemize}
  The set of all indexed heap configurations is denoted by $\IHC$.
\end{definition}

Here, the last two conditions ensure that the node $\vNull$, which represents the special location $\Null$, is unique --- even if summary edges are replaced by other indexed heap configurations as we will show in the following.


\begin{figure}[t]
    \center
    \input{pics/stackabstraction}
    \caption{Three indexed heap configurations modeling balanced binary trees}
    \label{fig:stackabstraction}
\end{figure}

\begin{example}\label{ex:indexed-hc}
Figure~\ref{fig:stackabstraction} shows three indexed heap configurations over the set of indices $\Index = \{ \Z, \iBot, S\}$.
The index of all edges labeled with fields or variables is set to $\iBot$ and thus omitted.
Summary edges are depicted as gray boxes labeled with the respective summary symbol ($B$) followed by their assigned index, e.g. $\Z\Z\Z\,\iBot$.
The numbered connections between summary edges and nodes represent their sequence of attached nodes.
Thus, the first attached node of the single summary edge of the leftmost graph is the $\Null$ node and the second attached node is the right child of the root of the depicted tree.
Finally, the sequence of external nodes is given by the numbers inside of nodes.
Hence, each of the graphs in Figure~\ref{fig:stackabstraction} has two external nodes: The $\Null$-node (1) and the root of the tree (2).
As we will see later, a summary edge $B$ with index $\Z\Z\Z\,\iBot$ represents all balanced binary trees of height three.
\end{example}


The semantics of summary edges is defined in terms of an extension of a classical graph rewriting mechanism. 
In this setting, we do not distinguish between isomorphic graphs, which are defined as follows:

\begin{definition}%[Isomorphic Indexed Hypergraphs]
\label{def:isomorphism}
  Let $\iH,\iK$ be indexed hypergraphs.
  Then $\iH$ and $\iK$ are \emph{isomorphic}, written $\iH \Iso \iK$, if and only if there exist
  bijective functions $f : \V_{\iH} \to \V_{\iK}$ and $g : \E_{\iH} \to \E_{\iK}$ such that
  \begin{itemize}
    \item for each $e \in \E_{\iH}$, $\Lab_{\iH}(e) = \Lab_{\iK}(g(e))$ and 
      $\Ind_{\iH}(e) = \Ind_{\iK}(g(e))$,  
    \item for each $e \in \E_{\iH}$, $f(\Att_{\iH}(e)) = \Att_{\iK}(g(e))$, and
    \item $f(\Ext_{\iH}) = \Ext_{\iK}$.
  \end{itemize}
\end{definition}


%\begin{example}\label{ex:isomorphism}
%\end{example}

\subsection{Indexed Hyperedge Replacement Grammars}\label{sec:ihrg}

Keeping in mind that all operations on graphs throughout this paper are to be read up to isomorphism, we now introduce \emph{indexed hyperedge replacement grammars} --- a lifting of indexed context-free string grammars~\cite{aho1968indexed} to graph grammars.
These grammars are then used to define the semantics of summary edges and guide concretization and abstraction.

\begin{definition}%[Indexed Hyperedge Replacement Grammar]
\label{def:ihrg}
Let $N$ and $T$ be disjoint finite sets of nonterminal and terminal symbols that are equipped with a ranking function $\Rank : N\cup T \to \Nats$.
Moreover, let $I$ be a finite set of index symbols and $\iVar \notin I$ be a dedicated \emph{index variable}.
An \emph{indexed hyperedge replacement grammar} (IG) is a finite set of production rules $\iG$ of the form
$%\begin{align*}
  \Rule{X,i}{\iH}
$ %\end{align*}
mapping a nonterminal $X \in N$ and an index sequence $i \in \I^{*} \iVar$ (or $i \in \I^{*})$ to an indexed graph $\iH$ over $N \cup T$ and $I \cup \{ \iVar \}$ (or $I$) such that $\Rank(X) = |\Ext_{\iH}|$.
\end{definition}

In our setting, the set of nonterminals is given by the set $\Sum$ of summary symbols.
In addition to that, we assume that every rule maps to an IHC that contains no program variables.

\begin{figure}[t]
    \center
    \input{pics/hrg_balanced_trees.tex}
    \caption{An indexed hyperedge replacement grammar for balanced binary trees}
    \label{fig:hrg_balanced_trees}
\end{figure}

Before we formally study indexed hyperedge replacement, we consider an example to illustrate how dynamic data structures are modeled by grammars.

\begin{example}\label{ex:ihrg}
Figure~\ref{fig:hrg_balanced_trees} depicts an indexed hyperedge replacement grammar $\iG$ over a single nonterminal $\B$ of rank two.
The set of terminals is $T = \{\ell,r,p\}$ and the set of indices is $\I = \{\Z,\iBot\}$.
$\iG$ consists of $6$ rules that each map nonterminal $\B$ and an index to a graph whose first external node is $\Null$ and whose second external node is the root of a small tree.
For simplicity, the index of all edges except from summary edges is $\iBot$ and thus omitted.

To gain some intuition, assume that nonterminal $\B$ represents binary trees.
Then, the rightmost rule in Figure~\ref{fig:hrg_balanced_trees} can be read as follows:
A single node whose whose children are both $\Null$ is a binary tree of height $0$.
It is thus represented by $\B$ (binary trees) and an index $\iBot$, where the end-of-index symbol $\iBot$ represents height $0$.
Conversely, this means that an edge labeled with $\B$ and an (empty) index $\iBot$ is mapped to a binary tree of height $0$.

Analogously, the leftmost rule in Figure~\ref{fig:hrg_balanced_trees} can be read as follows:
A tree (nonterminal $\B$) of height $1 + \iVar$, where $\iVar$ is a variable,  
can be composed of a tree of height one with two children that both are the root of a tree of height $\iVar$.
\end{example}

We now formalize the sets of graphs described by IGs.
In particular, this involves lifting common concepts from CFGs, such as derivations and languages, to IGs.
Recall that a CFG derivation replaces a nonterminal symbol by a finite string.
Similarly, an IG derivation consists of picking an edge, say $e$, that is labeled with a nonterminal $X$ and replacing it with a graph, say $\iK$.
However, since arbitrarily many nodes may be attached to an edge, we must define how the original graph and $\iK$ are glued into a single graph.
This is specified by the sequence of external nodes $\Ext_{\iK}$ that identifies each node attached to $e$ with a node of $\iK$ according to their position in $\Ext_{\iK}$ and $\Att(e)$.
Formally,

\begin{definition}%[Indexed Hyperedge Replacement]
        \label{def:ihr}
  Let $\iH,\iK$ be indexed hypergraphs over $N \cup T$ and $\I$ with pairwise disjoint sets of nodes and edges.
  Moreover, let $e \in \E_{\iH}$ be an edge such that $\Rank(\Lab_{\E_{\iH}}(e)) = |\Ext_{\iK}|$.
  Then the \emph{replacement} of $e$ in $\iH$ by $\iK$
  is given by $\Replace{\iH}{e}{\iK} = (\V,\E,\Att,\Lab,\Ind,\Ext)$, where
  \begin{align*}
          \V ~=~ & \V_{\iH} ~\cup~ \left( \V_{\iK} \setminus \Ext_{\iK} \right) 
                 &
          \E ~=~ & \underbrace{\left( \E_{\iH} \setminus \{ e \} \right)}_{=\,\E'} ~\cup~ \E_{\iK} \\
          %
          \Lab ~=~ & \left(\Proj{\Lab_{\iH}}{\E'}\right) ~\cup~ \Lab_{\iK}
                   &
          \Ind ~=~ & \left(\Proj{\Ind_{\iH}}{\E'}\right) ~\cup~ \Ind_{\iK} \\
          %
          \Att ~=~ & \left(\Proj{\Att_{\iH}}{\E'}\right) ~\cup~ \left( \textit{mod} \circ \Att_{\iK} \right)
                   &
          \Ext ~=~ & \Ext_{\iH}
  \end{align*}
  where $\textit{mod}$ replaces each external node by the corresponding node attached to $e$, i.e.
  $\textit{mod} = \{ \Elem{\Ext_{\iK}}{k} \mapsto \Elem{\Att_{\iH}(e)}{k} ~|~ 1 \leq k \leq |\Ext_{\iK}| \} \cup \{ v \mapsto v ~|~ v \in \V \setminus \Ext_{\iK} \}$.
\end{definition}

This is the standard definition of hyperedge replacement in which indices and edge labeled are treated the same (cf.~\cite{habel1992hyperedge}).
It is then tempting to define that an IG $\iG$ derives an IHC $\iK$ from an IHC $\iH$ if and only if 
there exists an edge $e \in \E_{\iH}$ and a rule $\Rule{\Lab_{\iH}(e),\Ind_{\iH}(e)}{\iR}$ such that
$\iK \Iso \Replace{\iH}{e}{\iR}$.
However, this notion of derivations is too weak to model complex data structures, such as balanced trees.
In particular, since an index is essentially just an edge label, we cannot apply a derivation if the index of an edge does not exactly match with an index occurring on the left-hand side of an IG rule.

To obtain more expressive grammars, we instead use IGs as a finite representation of infinitely many rules with different indices:
For example, assume an IG contains a rule $\Rule{\B,\Z\Z\iVar}{\iR}$.
Given an edge with label $\B$ and index $i = \Z\Z\Z\iBot$, an IG derivation may hide an arbitrary suffix, such as $\Z\iBot$, in the variable $\iVar$.
This yields an index $\Z\Z\iVar$ such that a derivation as defined naively above is possible.
After that, all occurrences of variable $\iVar$ are replaced by the hidden suffix again, i.e. $\iVar$ is replaced by $\Z\iBot$ in our example.

Towards a formal definition of IG derivations, we use two auxiliary definitions:
Given a set $M \subseteq T \cup N$, we write $\E_{\iH}^{M}$ to refer to all edges of $\iH$ that are labeled with a symbol in $M$, i.e. $\E_{\iH}^{M} = \{ e \in \E_{\iH} ~|~ \Lab_{\iH}(e) \in M \}$.
As for strings, we write $\Replace{\iH}{\iVar}{j}$ to replace all occurrences of symbol $\iVar$ in (the index function of) $\iH$ by $j$.\footnote{$\Replace{\iH}{\iVar}{j} = (\V_{\iH},\E_{\iH},\Att_{\iH},\Lab_{\iH},\Ind,\Ext_{\iH})$ with $\Ind = \{ \Replace{\Ind_{\iH}(e)}{\iVar}{j} ~|~ e \in \E_{\iH} \}$.}

\begin{definition}%[IG Derivation]
\label{def:derive}
Let $\iG$ be an IG and $\iH,\iK$ be indexed hypergraphs over $N \cup T$ and $\I$.
Then $\iG$ \emph{directly derives} $\iK$ from $\iH$, written $\iH \iDerive{\iG} \iK$,
if and only if either
\begin{itemize}
  \item there exists a rule $\Rule{X,i}{\iR} \in \iG$ and an edge $e \in \E_{\iH}^{\{X\}}$ such that
        $\Ind_{\iH}(e) = i$ and $\iK \Iso \Replace{\iH}{e}{\iR}$, or
  \item there exists a rule $\Rule{X,i\iVar}{\iR} \in \iG$, an edge $e \in \E_{\iH}^{\{X\}}$, and 
          a sequence $j \in \I^{*}$ such that $\Ind_{\iH}(e) = i \cdot j$ and $\iK \Iso \Replace{\iH}{e}{\Replace{\iR}{\iVar}{j}}$.
\end{itemize}
%Furthermore, the inverse of $\iDerive{\iG}$ is given by $\rDerive{\iG}$, i.e.
%$\iH \rDerive{\iG} \iK$ holds if and only if $\iK \iDerive{\iG} \iH$.
%The reflexive and transitive closure of $\iDerive{\iG}$ and $\rDerive{\iG}$ is denoted by $\iDerive{G}^{*}$ and $\rDerive{\iG}^{*}$, respectively.
\end{definition}

\begin{remark}\label{rem:increasing}
Throughout this paper  we assume that all rules of an IG are \emph{increasing}, i.e. for each rule $\Rule{X,i}{\iH}$ it holds that $|\V_{\iH}| + |\E_{\iH}| > \Rank(X)+1$.
This amounts to a syntactic check on all rules that easily discharged automatically.
\end{remark}


%\begin{remark}
%Algorithmically, an inverse derivation $\iH \rDerive{\iG} \iK$ corresponds to applying a rule $\Rule{X,i}{\iH}$ backwards, i.e. replacing a graph embedded in a given graph by a hyperedge.
%A formal definition is provided in Appendix~\ref{app:inverse-derivation}.
%\end{remark}

\begin{example}\label{ex:derive}
Let $\iG$ be the IG depicted in Figure~\ref{fig:hrg_balanced_trees}.
Then $\iG$ can derive the leftmost IHC $\iK$ in Figure~\ref{fig:stackabstraction} from the IHC $\iH$ in the middle of Figure~\ref{fig:stackabstraction}. 
To this end, the leftmost summary edge of $\iH$ is first replaced by the leftmost rule of $\iG$.
This introduces two new summary edges with index $\Z\iBot$ which are again replaced using the first rule of $\iG$.
Finally, the resulting summary edges with index $\iBot$ are all replaced according to the rightmost rule of $\iG$
to obtain the IHC $\iK$.
\end{example}

Similarly to CFGs, we then define the \emph{language} of an IG and an indexed heap configuration $\iH$ as the set of all graphs that can be derived from $\iH$ and that contain terminals only.
Analogously, the inverse language is the set of all indexed hypergraphs obtained from inverse derivations starting from a given graph, such that no further inverse derivation is possible.
Formally,

\begin{definition}\label{def:language}
The \emph{language} $\iL{\iG}$ and the \emph{inverse language} $\rL{\iG}$ of IG $\iG$ are
\begin{align*}
        \iL{\iG} : \IHC \to \PS{\IHC},~ \iH \mapsto\, & \{ \iK ~|~ \iH \iDerive{\iG}^{*} \iK ~\text{and}~ \E_{\iK} = \E_{\iK}^{T}\},
        ~\text{and} \\
\rL{\iG} : \IHC \to \PS{\IHC},~ \iH \mapsto\, & \{ \iK ~|~ \iH \rDerive{\iG}^{*} \iK ~\text{and}~ \iK \not\rDerive{\iG} \}.
\end{align*}
\end{definition}

\begin{example}\label{ex:language}
The IG $\iG$ depicted in Figure~\ref{fig:hrg_balanced_trees} models all balanced binary trees with additional parent pointers, where the height of said trees is depicted by the length of the initial index.
Hence, the language of $\iG$ and the IHC in the middle of Figure~\ref{fig:stackabstraction} is the set of all balanced binary trees, where the left child is the root of a balanced tree of height two and the right child is the root of a balanced tree of height three, respectively.
\end{example}

We conclude our introduction of IGs with a collection of useful properties.

\begin{theorem}%[IG Properties]
\label{thm:ig-props}
  Let $\iG$ be an IG and $\iH,\iK$ be indexed heap configurations. 
  Then the following properties hold:
  \begin{enumerate}
    \item $\iH \iDerive{\iG}^{*} \iK$ implies $\Lang{\iG}{\iK} \subseteq \Lang{\iG}{\iH}$.
    \item $\Lang{\iG}{\iH} = 
            \begin{cases}
                    \{ \iH \} &~\text{if}~ \neg \exists e \in \E_{\iH} : \Lab_{\iH}(e) \in N \\
                \bigcup_{\iH \iDerive{\iG} \iK} \Lang{\iG}{\iK} &~\text{otherwise.}
            \end{cases}$
    \item It is decidable whether $\Lang{\iG}{\iH} = \emptyset$ holds.
%    \item It is decidable whether $\Lang{\iG}{\iH} \subseteq \IHC$ holds.
    \item The inverse language $\iLang{\iG}{\iH}$ is non-empty and finite.
  \end{enumerate}
\end{theorem}

\begin{proof}
  See Appendix~\ref{app:ig-props}.
  \qed
\end{proof}

The first two properties show how IG derivations affect the language of IHCs and how the language of an IHC can be constructed incrementally using IG derivations.
Both properties are required in proving our analysis sound.
%
The third property allows to automatically check whether some graph without nonterminals can be derived from an IHC.
%The third property allows to automatically verify that the set of graphs described by the language of an IHC is useful.
%That is, it consists only of IHCs.
%%and it contains some IHC without summary edges, i.e. its language is non-empty.
%As we will use languages of IHCs for concretization, this means we can automatically discharge  that some heap configuration is actually captured by an IHC with summary edges.
%
%Conversely, we will use inverse languages for abstraction.
Finally, the last property ensures that constructing the inverse language of an IHC 
%by iteratively applying inverse derivations 
always terminates and yields a non-empty finite set.



==> concrete.tex <==
To set the stage for our analysis, we consider program states in the context of shape analysis to consist of a heap and a stack.
We assume the heap to consist of records with a finite number of \emph{reference fields} that are collected in $\Fields$. 
As such, we assume a storeless model that is agnostic of concrete memory addresses (cf.~\cite{rinetzky2005semantics}).
Since we disregard memory addresses, it is intuitive to model heaps as directed edge-labeled graphs:
Every record---including a special location $\Null$---is represented by a node and every pointer between two records is represented by a directed edge that is labeled with the respective field.
Apart from the heap, a program state is equipped with a \emph{stack} mapping program variables in $\Var$ to records.
We model the stack by adding special edges labeled with variables to the graph that are incident to the record stored in a variable.
%We model the stack as part of the graph by adding special edges that are labeled with the variable in question and incident to the variable's destination.
We allow edges to be incident to arbitrarily many nodes --- a feature that is needed later to define our abstract domain. 
Thus, we use \emph{hypergraphs} as the underlying formal model.

\begin{definition}%[Hypergraph]
\label{def:hypergraph}
  Let $S$ be a set equipped with a ranking function $\Rank : S \to \Nats$.
  A \emph{hypergraph} over $S$ is a tuple $\iH = \left(\V, \E, \Lab, \Att \right)$, where 
  \begin{compactitem}
  %\begin{itemize}
    \item $\V$ and $\E$ are finite sets of \emph{nodes} and \emph{hyperedges}, respectively, 
    \item $\Lab : \E \to S$ is a \emph{hyperedge labeling function}, and 
    \item $\Att : \E \to \V^{*}$ is an \emph{attachment function} respecting the rank of hyperedge labels, i.e. for all $e \in \E$, we have $\Rank(\Lab(e)) = |\Att(e)|$.
  %\end{itemize}
  \end{compactitem}
  %All hypergraphs over $S$ are collected in $\Graphs{S}$.
\end{definition}

Since only hypergraphs are considered in this paper, we do not distinguish between the terms graph and hypergraph nor between edge and hyperedge.
Furthermore, we often refer to the components of a graph $\iH$ by $\V_{\iH}$, $\E_{\iH}$, etc.

%\begin{figure}[t]
%  \center
%%  \input{pics/hc}
%  \scalebox{0.8}{
%  \input{pics/example1}
%  }
%  \caption{Graphs $\pIn$ (left) and $\pOut$ (right) modeling trees with parent pointers}
%  \label{fig:hc}
%\end{figure}

For our model of program states, we consider graphs over the set $\Var \,\cup\, \Fields$ of variables and fields, where we assign a rank of one to all variables and a rank of two to all fields, respectively.
%
%\begin{example}\label{ex:hypergraph}
%    As a running example, we consider binary trees with parent pointers.
%    Thus, unless explicitly stated otherwise, in all examples throughout this paper, the set of fields $\Fields$ consists of {\color{\lColor}\sL (eft)}, {\color{\rColor}\sR (ight)}, and {\color{\pColor}\sP (arent)}.
%    Two graphs modeling such trees are depicted in Figure~\ref{fig:hc}.
%    In our graphical notation, nodes are drawn as circles.
%    For the sake of readability, we draw multiple instances of the unique $\Null$--node, which is represented by a black circle.
%    Edges labeled with variables are drawn as diamonds connected to the single node they are attached to. 
%    Both graphs in Figure~\ref{fig:hc} contain four such edges that are labeled with $xp$, $x$, $t$ and $tl$, respectively.
%    Further, we draw edges labeled with fields (which are of rank two) as directed edges from the first to the second attached node. 
%    Consequently, if $\Att(e) = uv$, we call $e$ an \emph{outgoing edge} of $u$.
%    The label of each edge is indicated by the respective color.
%    %For readability purposes, we illustrate fields by colors. %the fields have been omitted in Figure~\ref{fig:hc}.
%    %$Their assignment to each of the directed edges should be clear from the context.
%    %For example, the edge from the root of the tree to the $\Null$--node is labeled with \sP, because the root of a binary tree has no parent.
%\end{example}
%
%Note that 
Some graphs do not model proper program states.
For instance, consider a node with two outgoing edges labeled with the same field.
This corresponds to a record having the same pointer pointing to different locations, which is clearly invalid.
We thus restrict ourselves to graphs representing program states (various examples are found in Section~\ref{sec:overview}): %, defined as follows:

\begin{definition}%[Heap Configuration]
\label{def:heapconf}
 A \emph{heap configuration} (HC) is a graph $\iH$ over a set containing $\Var \cup \Fields$ such that
 % \begin{itemize}
 %   \item 
 (1) every variable $x \in \Var$ occurs at most once in $\iH$,
 %   \item 
 (2) for each field $f \in \Fields$, every node in $\iH$ has at most one outgoing edge labeled with $f$\footnote{i.e. for all $v \in \V_{\iH}$ there is at most one $e \in \E_{\iH}$ with $\Att_{\iH}(e)(1) = v$ and $\Lab_{\iH}(e) = f$.}
 %   \item 
 (3) there is a unique node $\vNull$ without outgoing edges labeled with fields.
 % \end{itemize}
  The set of all heap configurations is denoted by $\HC$.
\end{definition}

%\begin{example}\label{ex:heapconf}
%  Both graphs depicted in Figure~\ref{fig:hc} are heap configurations if all black nodes are considered as the single node $\vNull$.
%  %The graph in Figure~\ref{fig:hc} is \emph{not} a heap configuration, because it contains two edges labeled with the same variable $x$.
%  %We obtain a heap configuration if one of these two edges is removed.
%\end{example}


\todo[inline]{
To what extend do we need a programming language and concrete semantics?
}

%For the sake of concreteness, 
%Since our focus lies on the abstract domain, we present our analysis in terms of 
%a small heap-manipulating programming language.
%%Note that we actually support %our analysis %implementation supports 
%The analysis actually supports
%a richer set of programming language features, such as %(potentially recursive) 
%procedure calls, that have been omitted to improve readability. %to keep the presentation simple. %to improve readability.
%For an in-depth treatment on %how to incorporate
%incorporating recursion %recursive procedures 
%into our analysis, we refer the interested reader to~\cite{DBLP:conf/gg/JansenN14}.
%
%%While our analysis is independent of a specific programming language, we present it in terms of a small heap-manipulating language for the matter of concreteness.
%Let $x$ be a variable taken from $\Var$ and $f \in \Fields$ be a field. 
%Then the syntax of \emph{programs} $\Progs$ ($\pP$), \emph{Boolean expressions} $\BExps$ ($\pB$), and \emph{pointer expressions} $\PExps$ ($\pE$) is defined by the 
%following
%context-free grammar: 
%%in Figure~\ref{fig:syntax} below:
%%
%%\begin{figure}[h]
%{\small
%\begin{align*}
%\pP ~::=~ &
%\Ass{x}{\pE} \,|\,
%\Ass{\F{x}{f}}{\pE} \,|\,
%\New{x} \,|\,
%\Seq{\pP}{\pP} 
%\,|\, \Skip
%%\tag{$\Progs$} 
% \,|\,
%\Ite{\pB}{\pP}{\pP} \,|\,
%\WhileDo{\pB}{\pP}
%\\
%\pB ~::=~ & 
%\Equals{\pE}{\pE} \,|\,
%\Con{\pB}{\pB} \,|\,
%\Not{\pB}
%%\tag{$\BExps$}
%%\\
%\qquad\qquad\quad
%\pE ~::=~ 
%\Null \,|\,
%x  \,|\,
%\F{x}{f} 
%%\tag{$\PExps$}
%\end{align*}
%}
%%\caption{Syntax of $\Progs$-programs}
%%\label{fig:syntax}
%%\end{figure}
%%
%The meaning of $\Progs$-programs is straightforward.
%For instance, %an assignment 
%$\Ass{\F{x}{f}}{\Null}$ sets the $f$-field of the record referenced by variable $x$ to %the location 
%$\Null$.
%%
%\begin{figure}[t]
%\begin{align*}
%& \PSem{\Ass{x}{\pE}} =
%\SetVar{x}{\ESem{\pE}}
%\qquad
%%
%\PSem{\Ass{\F{x}{f}}{\pE}} =
%\SetField{x}{f}{\ESem{\pE}}
%\\
%%
%& \PSem{\New{x}} =
%\AddVar{x}
%\qquad
%\PSem{\Skip} =
%\Id{\HC}
%%
%\qquad
%%
%\PSem{\Seq{\pP_1}{\pP_2}} =
%\PSem{\pP_1} \FComp \PSem{\pP_2}
%%
%\\
%& \PSem{\Ite{\pB}{\pP_1}{\pP_2}} =
%\SemIte{\BSem{\pB}}{\PSem{\pP_1}}{\PSem{\pP_2}}
%%
%\\
%%
%& \PSem{\WhileDo{\pB}{\pP}} =
%\Lfp \, Y \,.\, \left( 
%%Y \mapsto \PSem{\Ite{\pB}{\Seq{\pP}{Y}}{\Skip}} 
%Y \mapsto 
%\SemIte{\BSem{\pB}}{\PSem{\pP_1}\FComp Y}{\PSem{\Skip}}
%\right)
%%
%\end{align*}
%%\begin{align*}
%%\PSem{\Ass{x}{\pE}} ~=~ & 
%%\SetVar{x}{\ESem{\pE}}
%%\\
%%%
%%\PSem{\Ass{\F{x}{f}}{\pE}} ~=~ & 
%%\SetField{x}{f}{\ESem{\pE}}
%%\\
%%%
%%\PSem{\New{x}} ~=~ &
%%\AddVar{x}
%%\\
%%\PSem{\Skip} ~=~ &
%%\Id{\HC}
%%\\
%%\PSem{\Ite{\pB}{\pP_1}{\pP_2}} ~=~ &
%%\SemIte{\BSem{\pB}}{\PSem{\pP_1}}{\PSem{\pP_2}}
%%\\
%%%
%%\PSem{\Seq{\pP_1}{\pP_2}} ~=~ &
%%\PSem{\pP_1} \FComp \PSem{\pP_2}
%%\\
%%%
%%\PSem{\WhileDo{\pB}{\pP}} ~=~ &
%%\Lfp \, Y \,.\, \left( Y \mapsto \PSem{\Ite{\pB}{\Seq{\pP}{Y}}{\Skip}} \right)
%%%
%%\end{align*}
%\caption{
%The semantics of $\Progs$-programs. 
%$\ESem{\pE}$ is a partial function that evaluates expression $\pE$ for a given HC $\iH$ to a corresponding node in $\iH$.
%The semantics of Boolean conditions $\pB$ is given by the partial function $\BSem{\pB} : \HC \to \{\True,\False\}$. 
%Further, the auxiliary functions $\SetVar{x}{\ESem{\pE}}$, $\SetField{x}{f}{\ESem{\pE}}$, and $\AddVar{x}$ are HC transformers of type $\HC \to \HC$ that (re)set variable $x$ to node $\ESem{\pE}$, (re)set the edge labeled with $f$ from the node $\ESem{x}$ to node $\ESem{\pE}$, and add a new node and assign $x$ to it, respectively.
%As is standard, the semantics of loops is defined as a least fixed-point, denoted by $\Lfp$.
%Formal definitions of all auxiliary functions are provided in Appendix~\ref{app:concrete}.
%}
%\label{fig:semantics}
%\end{figure}
%%
%Formally, the semantics of $\Progs$-programs is given by a function 
%%\[ \PSem{.} : \Progs \to \HC \to \HC \]
%$\PSem{.} : \Progs \to \HC \to \HC$
%that takes a program $P$ and a program state, i.e. an HC $\iH$, and yields an HC capturing the effect of executing $P$ on $\iH$.
%In Figure~\ref{fig:semantics} the transformer $\PSem{.}$ is defined inductively on the structure of $\Progs$-programs.
%%
%For example, the semantics of an assignment $\Ass{\F{x}{f}}{y}$ first computes the nodes $\ESem{x}$ and $\ESem{y}$ attached to variable edges $x$ and $y$, respectively.
%After that, existing outgoing edges of $\ESem{x}$ labeled with $f$ are removed.
%Finally, a new edge $e$ from $\ESem{x}$ to $\ESem{y}$ with label $f$ is added.
%The semantics of the control-flow structures is standard (cf.~\cite{nielson2007semantics}).
%
%%\begin{example}\label{ex:semantics}
%%        Consider the $\Progs$-program $\pEx$ shown in Figure~\ref{fig:program-rotateLeft}.
%%        As an input, $\pEx$ takes a variable $x$ pointing to a node in a binary tree with a right child.
%%%        It then performs a left rotation of the tree with root $x$ and finally sets $x$ to the root of the rotated tree, i.e. the original right child of $x$.
%%%        All other introduced variables are set to $\Null$.
%%        Figure~\ref{fig:hc} (left) illustrates an input graph in which $\pEx$ has already been executed up to the line marked with $\texttt{(*)}$. 
%%        %Assume we are given the graph $\pIn$ in Figure~\ref{fig:hc} (left) as an input.
%%        Then the graph $\pOut$ in Figure~\ref{fig:hc} (right) depicts the HC after the remainder of $\pEx$ has been executed on $\pIn$.
%%        %The result of executing the whole program $\pEx$ on $\pIn$, i.e. $\PSem{\pEx}(\pIn)$, is the same graph as $\pOut$ except that the variables $t$ and $x$ are switched and afterwards all variable edges other than $x$ are set to $\Null$. That is, they are connected to the (black) node $\vNull$.
%%\end{example}
%%%
%%\begin{figure}[t]
%%\centering
%%\begin{align*}
%%        1\quad &
%%        \texttt{//}~ x,\F{x}{\fR} \neq \Null 
%%        & 6\quad &
%%        \Ass{\F{t}{\fP}}{xp}; \\
%%        %
%%        2\quad &
%%        \Ass{t}{\F{x}{\fR}}; 
%%        & 7\quad &
%%        \Ass{\F{x}{\fR}}{tl}; \\
%%        %
%%        3\quad &
%%        \Ass{tl}{\F{t}{\fL}}; 
%%        & 8\quad &
%%        \Ass{\F{x}{\fP}}{t}; \\
%%        %
%%        4\quad &
%%        \Ass{xp}{\F{x}{\fP}}; ~ \texttt{// (*)} 
%%        & 9\quad &
%%        \Ass{\F{t}{\fL}}{x}; \\
%%        %
%%        5\quad &
%%        \IF{\neg (\Equals{xp}{\Null})} \{ \Ass{\F{xp}{\fR}}{t}; \} 
%%        & 10\quad &
%%        \IF{\neg (\Equals{tl}{\Null})} \{ \Ass{\F{tl}{\fP}}{x}; \}
%%\end{align*}
%%\caption{Program $\pEx$}
%%\label{fig:program-rotateLeft}
%%\end{figure}
%%


==> excursus.tex <==

For our abstract domain, we equip heap configurations with additional edges
that act as placeholders for possibly infinite sets of graphs, such as all binary trees.
The formal semantics of these edges is defined by a \emph{hyperedge replacement grammar} (HRG) --- a well-established formalism for context-free graph rewriting~\cite{habel1992hyperedge}.
%This approach is equivalent to a fragment of symbolic heap separation logic with inductive predicates~\cite{berdine2005symbolic}, where the semantics of predicates is defined by a system of inductive definitions (cf.~\cite{jansen2014generating}).
%
However, the context-free nature of HRGs %hyperedge replacement grammars 
means that some complex data structures, such as \emph{balanced} binary trees, are not expressible.
Hence, we introduce a more powerful formalism: \emph{indexed hyperedge replacement grammars} (IG).
These grammars are obtained from lifting indexed string grammars --- a classical extension of CFGs introduced in~\cite{aho1968indexed} --- to graph grammars.

As the name suggests, we first extend graphs by \emph{indices}.
Throughout this section, we fix a finite non-empty set of index symbols $\I$.
%that includes the \emph{end-of-index} symbol $\iBot$.
Moreover, let $N$ and $T$ be disjoint finite sets of \emph{nonterminals} and \emph{terminals} that are equipped with a ranking function $\Rank : (N \cup T) \to \Nats$.
We then additionally assign an index, i.e. a finite, non-empty sequence over $\I$, to each edge:
\begin{definition}%[Indexed Hypergraph]
\label{def:indexed-hg}
   An \emph{indexed hypergraph} over the sets $N \cup T$ and $\I$ is a tuple
   $\iH = (\V,\E,\Lab,\Att,\Ind,\Ext)$, where
    %\begin{compactitem}
   \begin{itemize}
     \item $(\V,\E,\Lab,\Att)$ is a hypergraph over $N \cup T$ according to Definition~\ref{def:hypergraph}, 
     \item $\Ind : E \to \I^{+}$ assigns an index to each edge in $\E$, and
     \item $\Ext \in \V^{*}$ is a (possibly empty) repetition-free sequence of \emph{external nodes}.
    %\end{compactitem}
    \end{itemize}
   %The set of all indexed hypergraphs over $S$ and $\I$ is $\IGraphs{S}{\I}$.
\end{definition}

External nodes are needed to define derivations %of graph grammars %in the following 
(cf. Definition~\ref{def:ihr}).

\todo[inline]{Example?!}

%\begin{figure}[b]
%    \center
%    \scalebox{0.8}{
%    \input{pics/example2}
%    }
%    \caption{Three indexed graphs. From left to right: $\iH_{\textit{left}}$, $\iH_{\textit{mid}}$, and $\iH_{\textit{right}}$}
%    \label{fig:stackabstraction}
%\end{figure}
%
%\begin{example}\label{ex:indexed-hc}
%Figure~\ref{fig:stackabstraction} illustrates three indexed graphs $\iH_{\textit{left}}$, $\iH_{\textit{mid}}$, and $\iH_{\textit{right}}$
%over the set of nonterminals $N = \{\B\}$, terminals $T = \Fields = \{\fL,\fR,\fP\}$ and indices $\I = \{\Z,\iBot\}$.
%We draw edges labeled with nonterminals as gray boxes that contain their label and their assigned index, such as $\Z\iBot$.
%The sequence of attached nodes of these edges is given by the numbered connections.
%For instance, the first attached node of every edge labeled with $\B$ is the black node representing $\Null$.
%Furthermore, the index of all edges with labels from $T$ is set to $\iBot$ and thus omitted.
%Finally, the sequence of external nodes is given by the numbers inside of nodes.
%Hence, each of the graphs in Figure~\ref{fig:stackabstraction} has two external nodes: The $\Null$-node (1) and the root of a tree-like graph (2).
%%As we will see later, a summary edge $B$ with index $\Z\Z\Z\,\iBot$ represents all balanced binary trees of height three.
%\end{example}

As it is common in graph rewriting, we do not distinguish between isomorphic graphs.
Thus, all sets of graphs in this paper are to be understood up to isomorphism. % $\Iso$.
\footnote{A formal definition of graph isomorphism is found in Appendix~TODO.}
%
%Formally, two indexed graphs $\iH$ and $\iK$ are \emph{isomorphic}, written $\iH \Iso \iK$, iff there exist %if and only if there exist
%  bijective functions $f : \V_{\iH} \to \V_{\iK}$, $g : \E_{\iH} \to \E_{\iK}$ such that
%  \begin{itemize}
%    \item for each $e \in \E_{\iH}$, $\Lab_{\iH}(e) = \Lab_{\iK}(g(e))$ and 
%      $\Ind_{\iH}(e) = \Ind_{\iK}(g(e))$,  
%    \item for each $e \in \E_{\iH}$, $f(\Att_{\iH}(e)) = \Att_{\iK}(g(e))$, and
%          $f(\Ext_{\iH}) = \Ext_{\iK}$.
%    %\item $f(\Ext_{\iH}) = \Ext_{\iK}$.
%  \end{itemize}
%
%\begin{definition}%[Isomorphic Indexed Hypergraphs]
%\label{def:isomorphism}
%  Let $\iH,\iK$ be indexed hypergraphs.
%  Then $\iH$ and $\iK$ are \emph{isomorphic}, written $\iH \Iso \iK$, if and only if there exist
%  bijective functions $f : \V_{\iH} \to \V_{\iK}$ and $g : \E_{\iH} \to \E_{\iK}$ such that
%  \begin{itemize}
%    \item for each $e \in \E_{\iH}$, $\Lab_{\iH}(e) = \Lab_{\iK}(g(e))$ and 
%      $\Ind_{\iH}(e) = \Ind_{\iK}(g(e))$,  
%    \item for each $e \in \E_{\iH}$, $f(\Att_{\iH}(e)) = \Att_{\iK}(g(e))$, and
%    \item $f(\Ext_{\iH}) = \Ext_{\iK}$.
%  \end{itemize}
%\end{definition}
Keeping this in mind, we now introduce indexed hyperedge replacement grammars.
These grammars guide concretization and abstraction of our analysis, which is presented subsequently in Section~\ref{sec:analysis}.


\begin{definition}%[Indexed Hyperedge Replacement Grammar]
\label{def:ihrg}
Let $\iVar$ be a dedicated \emph{index variable} that is \emph{not} contained in the set of index symbols $\I$.
An \emph{indexed hyperedge replacement grammar} (IG) is a finite set of rules $\iG$ of the form
$%\begin{align*}
  \Rule{X,\sigma}{\iH}
$ %\end{align*}
mapping a nonterminal $X \in N$ and an index $\sigma \in \I^{*} (I \cup \{\iVar\})$ to an indexed graph $\iH$ over $N \cup T$ and $I \cup \{ \iVar \}$ such that $\Rank(X) = |\Ext_{\iH}|$.
Moreover, if $\sigma$ does not contain the variable $\iVar$ then $\iH$ does not contain $\iVar$ either, i.e.
$\Ind_{\iH}(\E_{\iH}) \subseteq \I^{+}$.
\end{definition}


\begin{figure}[t]
    \center
    \scalebox{0.8}{
    \input{pics/hrg_balanced_trees.tex}
    }
    \caption{An indexed hyperedge replacement grammar for balanced binary trees}
    \label{fig:hrg_balanced_trees}
\end{figure}

%Before we formally study derivations and languages of IGs, we consider an example to illustrate how IGs can be applied to model complex data structures.

\begin{example}\label{ex:ihrg}
Figure~\ref{fig:hrg_balanced_trees} depicts an IG $\iG$ %over a single nonterminal $\B$ of rank two.
%The set of terminals is $T = \{\fL,\fR,\fP\} \subseteq \Fields$ and the set of indices is $\I = \{\Z,\iBot\}$.
consisting of 
%$\iG$ consists of 
six rules that each map to a graph whose first external node is $\Null$ and whose second external node is the root of a tree-like graph.
Again, the indices of all edges that are not labeled with $\B$ are set to $\iBot$ and thus omitted.
%
%To gain some intuition, assume that nonterminal $\B$ represents binary trees.
%Then, the rightmost rule in Figure~\ref{fig:hrg_balanced_trees} can be read as follows:
%A single node whose whose children are both $\Null$ is a binary tree of height $0$.
%It is thus represented by $\B$ (binary trees) and an index $\iBot$, where the end-of-index symbol $\iBot$ represents height $0$.
%Conversely, this means that an edge labeled with $\B$ and an (empty) index $\iBot$ is mapped to a binary tree of height $0$.
%
%Analogously, the leftmost rule in Figure~\ref{fig:hrg_balanced_trees} can be read as follows:
%A tree (nonterminal $\B$) of height $1 + \iVar$, where $\iVar$ is a variable,  
%can be composed of a tree of height one with two children that both are the root of a tree of height $\iVar$.
\end{example}

The sets of graphs modeled by IGs are defined similarly to languages of CFGs.
%To interpret how IGs model sets of graphs, we now lift common notions from CFGs to IGs.
%To formalize the sets of graphs modeled by IGs, we now lift common concepts of CFGs to IGs.
Recall from Section~\ref{sec:preli} that a CFG derivation replaces a nonterminal by a finite string.
Similarly, an IG derivation replaces an edge, say $e$, that is labeled with a nonterminal by a finite graph, say $\iK$.
However, since arbitrarily many nodes may be attached to an edge, we have to clarify how the original graph and $\iK$ are glued together.
This is specified by the external nodes of $\iK$ that identify each node attached to $e$ with a node of $\iK$.
Formally,

\begin{definition}%[Indexed Hyperedge Replacement]
        \label{def:ihr}
  Let $\iH,\iK$ be indexed graphs over $N \cup T$ and $\I$ with pairwise disjoint sets of nodes and edges.
  Moreover, let $e \in \E_{\iH}$ be an edge such that $\Rank(\Lab_{\E_{\iH}}(e)) = |\Ext_{\iK}|$.
  Then the \emph{replacement} of $e$ in $\iH$ by $\iK$
  is given by $\Replace{\iH}{e}{\iK} = (\V,\E,\Att,\Lab,\Ind,\Ext)$, where
  \begin{align*}
          \V ~=~ & \V_{\iH} ~\cup~ \left( \V_{\iK} \setminus \Ext_{\iK} \right) 
                 &
          \E ~=~ & \underbrace{\left( \E_{\iH} \setminus \{ e \} \right)}_{=\,\E'} ~\cup~ \E_{\iK} \\
          %
          \Lab ~=~ & \left(\Proj{\Lab_{\iH}}{\E'}\right) ~\cup~ \Lab_{\iK}
                   &
          \Ind ~=~ & \left(\Proj{\Ind_{\iH}}{\E'}\right) ~\cup~ \Ind_{\iK} \\
          %
          \Att ~=~ & \left(\Proj{\Att_{\iH}}{\E'}\right) ~\cup~ \left( \Att_{\iK} \FComp \textit{mod} \right)
                   &
          \Ext ~=~ & \Ext_{\iH}
  \end{align*}
  where $\textit{mod}$ replaces each external node by the corresponding node attached to $e$, i.e.
  $\textit{mod} = \{ \Elem{\Ext_{\iK}}{k} \mapsto \Elem{\Att_{\iH}(e)}{k} ~|~ 1 \leq k \leq |\Ext_{\iK}| \} \cup \{ v \mapsto v ~|~ v \in \V \setminus \Ext_{\iK} \}$.
\end{definition}

This is the standard definition of hyperedge replacement in which indices and edge labels are treated the same (cf.~\cite{habel1992hyperedge}).
It is then tempting to define that an IG $\iG$ derives $\iK$ from $\iH$ if and only if 
there exists an edge $e \in \E_{\iH}$ and a rule $(\Rule{\Lab_{\iH}(e),\Ind_{\iH}(e)}{\iR}) \in \iG$ such that
$\iK$ is isomorphic to $\Replace{\iH}{e}{\iR}$.
%$\iK \Iso \Replace{\iH}{e}{\iR}$.
However, this notion is too weak to model balanced trees.
In particular, since an index is treated as just another label, we cannot apply a derivation if the index of an edge does not exactly match an index on the left-hand side of an IG rule.

Instead, we use %consider 
a finite prefix of indices in derivations and hide the remainder in the variable $\iVar$. %, if present.
For example, assume an IG contains a rule $\Rule{\B,\Z\Z\iVar}{\iR}$.
Given an edge with label $\B$ and index $\sigma = \Z\Z\Z\iBot$, an IG derivation may then hide $\Z\iBot$ in $\iVar$.
This yields an index $\Z\Z\iVar$ such that a derivation as defined naively above is possible.
Finally,
%After that, 
all occurrences of %variable 
$\iVar$ are replaced 
by the hidden suffix $\Z\iBot$ again. 

To formalize indexed derivations, two auxiliary definitions are needed:
Given a set $M \subseteq T \cup N$, we write $\E_{\iH}^{M}$ to refer to all edges of $\iH$ that are labeled with a symbol in $M$, i.e. $\E_{\iH}^{M} = \{ e \in \E_{\iH} ~|~ \Lab_{\iH}(e) \in M \}$.
As for strings, we write $\Replace{\iH}{\iVar}{\rho}$ to replace all occurrences of $\iVar$ in (the index function of) $\iH$ by $\rho$.\footnote{$\Replace{\iH}{\iVar}{\rho} = (\V_{\iH},\E_{\iH},\Att_{\iH},\Lab_{\iH},\Ind,\Ext_{\iH})$ with $\Ind = \{ \Replace{\Ind_{\iH}(e)}{\iVar}{\rho} ~|~ e \in \E_{\iH} \}$.}

\begin{definition}%[IG Derivation]
\label{def:derive}
Let $\iG$ be an IG and $\iH,\iK$ be indexed hypergraphs over $N \cup T$ and $\I$.
Then $\iG$ \emph{directly derives} $\iK$ from $\iH$, written $\iH \iDerive{\iG} \iK$,
if and only if either
\begin{itemize}
  \item there exists a rule $(\Rule{X,\sigma}{\iR}) \in \iG$ and an edge $e \in \E_{\iH}^{\{X\}}$ such that
        $\Ind_{\iH}(e) = \sigma$ and $\iK$ is isomorphic to $\Replace{\iH}{e}{\iR}$, or 
  \item there exists a rule $(\Rule{X,\sigma\iVar}{\iR}) \in \iG$, an edge $e \in \E_{\iH}^{\{X\}}$, and 
          a sequence $\rho \in \I^{+}$ such that $\Ind_{\iH}(e) = \sigma \rho$ and $\iK$ is isomorphic to $\Replace{\iH}{e}{\Replace{\iR}{\iVar}{\rho}}$.
\end{itemize}
%Furthermore, the inverse of $\iDerive{\iG}$ is given by $\rDerive{\iG}$, i.e.
%$\iH \rDerive{\iG} \iK$ holds if and only if $\iK \iDerive{\iG} \iH$.
%The reflexive and transitive closure of $\iDerive{\iG}$ and $\rDerive{\iG}$ is denoted by $\iDerive{G}^{*}$ and $\rDerive{\iG}^{*}$, respectively.
\end{definition}

%\begin{remark}\label{rem:increasing}
        To simplify the technical development we assume throughout this paper that all rules of an IG $\iG$ are \emph{increasing}, i.e. for each rule $(\Rule{X,\sigma}{\iH}) \in \iG$ it holds that $|\V_{\iH}| + |\E_{\iH}| > \Rank(X)+1$.
This amounts to a syntactic check on all rules that is easily discharged automatically.
%\end{remark}


%\begin{remark}
%Algorithmically, an inverse derivation $\iH \rDerive{\iG} \iK$ corresponds to applying a rule $\Rule{X,i}{\iH}$ backwards, i.e. replacing a graph embedded in a given graph by a hyperedge.
%A formal definition is provided in Appendix~\ref{app:inverse-derivation}.
%\end{remark}

\todo[inline]{Example?!}
%\begin{example}\label{ex:derive}
%Recall the graphs $\iH_{\textit{left}}$, $\iH_{\textit{mid}}$, and $\iH_{\textit{right}}$ from Figure~\ref{fig:stackabstraction} (p. \FIGNINEPAGE).
%The IG $\iG$ %depicted 
%in Figure~\ref{fig:hrg_balanced_trees} derives $\iH_{\textit{mid}}$ from $\iH_{\textit{right}}$ by applying the rightmost rule of $\iG$ to the edge with label $\B$ and index $\iBot$.
%That is, $\iH_{\textit{right}} \iDerive{\iG} \iH_{\textit{mid}}$.
%Further, we have $\iH_{\textit{mid}} \iDerive{\iG} \iH_{\textit{left}}$ as we can apply the third rule of $\iG$ in Figure~\ref{fig:hrg_balanced_trees} to the single $\B$-labeled edge in $\iH_{\textit{mid}}$.
%Conversely, this means that $\iH_{\textit{left}} \rDerive{\iG}^{*} \iH_{\textit{right}}$. 
%\end{example}

Similarly to CFGs, we define the \emph{language} of an IG and an indexed graph $\iH$ as the set of all graphs that can be derived from $\iH$ and that contain terminal edge labels only.
Conversely, the inverse language of $\iH$ is obtained by exhaustively applying inverse derivations to $\iH$.
Formally,
%is the set of all indexed graphs 
%obtained from inverse derivations of  a given graph until %, such that 
%no further inverse derivation is possible.
%Formally,

\begin{definition}\label{def:language}
The \emph{language} $\iL{\iG}$ and the \emph{inverse language} $\rL{\iG}$ of IG $\iG$ are given by the following functions mapping indexed graphs to sets of indexed graphs:
%such that for all $\iH$:
\begin{align*}
        \iL{\iG}(\iH) ~=~ & \{ \iK ~|~ \iH \iDerive{\iG}^{*} \iK ~\text{and}~ \E_{\iK} = \E_{\iK}^{T}\},
        ~\text{and} \\
        \rL{\iG}(\iH) ~=~ & \{ \iK ~|~ \iH \rDerive{\iG}^{*} \iK ~\text{and}~ \iK \nrDerive{\iG} \}.
\end{align*}
\end{definition}

\todo[inline]{Example?!}

%\begin{example}\label{ex:language}
%Again, we consider the IG $\iG$ in Figure~\ref{fig:hrg_balanced_trees} (p. \GRAMMARPAGE) and the graphs $\iH_{\textit{left}}$ and $\iH_{\textit{right}}$ in Figure~\ref{fig:stackabstraction} (p. \FIGNINEPAGE).
%We have $\iH_{\textit{right}} \in \rL{\iG}(\iH_{\textit{left}})$, because $\iH_{\textit{right}} \rDerive{\iG}^{*} \iH_{\textit{left}} \nrDerive{\iG}$.
%However, $\iH_{\textit{left}} \notin \iL{\iG}(\iH_{\textit{right}})$ due to the fact that $\iH_{\textit{left}}$ still contains edges labeled with nonterminals.
%%Again, we consider the IG $\iG$ in Figure~\ref{fig:hrg_balanced_trees} (p. \GRAMMARPAGE) and the graphs $\pIn$  in Figure~\ref{fig:hc} (without variables and external node $\vNull$) and $\iH_{\textit{left}}, \iH_{\textit{right}}$ in  Figure~\ref{fig:stackabstraction} (p. \FIGNINEPAGE).
%%Then $\pIn \in \iL{\iG}(\iH_{\textit{right}})$, because $\iH_{\textit{right}} \iDerive{\iG}^{*} \iH_{\textit{left}}$ and $\iH_{\textit{left}} \iDerive{\iG}^{*} \pIn$.
%%In particular, note that no inverse derivation of $\iG$ is applicable to $\iH_{\textit{right}}$ due to the indices.
%%Consequently, we have $\iH_{\textit{right}} \in \rL{\iG}(\iH_{\textit{left}})$.
%
%In this example, $\iG$ uses indices over $\iBot$ and $\Z$ to model a counter, where $\iBot$ represents the initial value zero and each $\Z$ represents an increment.
%The value of such a counter then corresponds to the height of all balanced binary trees that can be derived from an edge with label $B$.
%For instance, an edge with label $\B$ and index $\Z\Z\Z\iBot$ represents the set of all balanced binary trees of height three. 
%\end{example}

We conclude our introduction of IGs with a collection of useful properties.

\begin{theorem}%[IG Properties]
\label{thm:ig-props}
  Let $\iG$ be an IG and $\iH$ be an indexed graph over $N \cup T$. Then:
  \begin{enumerate}
    \item $\iH \iDerive{\iG}^{*} \iK$ implies $\Lang{\iG}{\iK} \subseteq \Lang{\iG}{\iH}$.
    \item $\Lang{\iG}{\iH} = 
            \begin{cases}
                    \{ \iH \} &~\text{if}~ \neg \exists e \in \E_{\iH} : \Lab_{\iH}(e) \in N \\
                \bigcup_{\iH \iDerive{\iG} \iK} \Lang{\iG}{\iK} &~\text{otherwise.}
            \end{cases}$
    \item It is decidable whether $\Lang{\iG}{\iH} = \emptyset$ holds.
    \item The inverse language $\iLang{\iG}{\iH}$ is non-empty and finite.
  \end{enumerate}
\end{theorem}

%\begin{proof}
%  See Appendix~\ref{app:ig-props}. \qed
%\end{proof}

The first property shows how IG derivations affect the language of indexed graphs.
The second property illustrates how the language of an indexed graph can be constructed incrementally using IG derivations.
Both properties are used to prove our analysis sound.
%
The third property allows to verify that the language of an IG covers at least some graph.
%
Finally, the last property ensures that constructing the inverse language of an indexed graph terminates. % and results in a non-empty finite set.
%


==> pics/dll_critical.tex <==
\begin{figure}[t]
\center
\scalebox{0.9}{
\tikzdefault{
    \location{v1}{}{}
    \location{v2}{right of = v1}{}
    \location{v3}{right of = v2}{}

    \nonterminal{L}{right}{v3}{\texttt{DLL}}

    \location{v4}{right of = L}{}
    \location{n1}{left of = v1}{}
    %\nil{n1}{left of = v1}
    \nil{n2}{right of = v4}


    \lpointer{v1}{bend left}{e0}{n1}{prev}{below}
    \lpointer{v1}{bend left}{e1}{v2}{next}{above}
    \lpointer{v2}{bend left}{e2}{v1}{prev}{below}
    \lpointer{v2}{bend left}{e3}{v3}{next}{above}
    %\lpointer{v3}{bend left}{e4}{v2}{prev}{below}
%    \lpointer{v4}{bend left}{e5}{n2}{next}{above}
    %\lpointer{v3}{bend left}{e5}{v4}{next}{above}
    %\lpointer{v4}{bend left}{e6}{v3}{prev}{below}

    \tentacleB{L}{1,5}{n2}{bend right}
    \tentacleB{L}{2}{v2}{bend left}
    \tentacle{L}{3}{v3}{}
    \tentacle{L}{4}{v4}{}

    \node[below of = n2, node distance=6mm] (dummyB) {};

      \begin{pgfonlayer}{background}
              \filldraw [line width=6mm,join=round,black!10]
              (e1.north -| n2.east) rectangle (dummyB.south -| v1);
              \filldraw [line width=4mm,join=round,black!20]
              (e1.north  -| v3.east)  rectangle (e0.south  -| n1.west);
              \filldraw [line width=4mm,join=round,black!20]
              (n2.north  -| n2.east)  rectangle (n2.south  -| n2.west);
      \end{pgfonlayer}

}
}
\caption{
    An IHC modeling doubly-linked list segments with two overlapping embeddings of rules of the IG in Figure~\ref{fig:hrg:dll}.
    One embedding (dark) corresponds to the first rule. The other embedding corresponds to the second rule.
}
\label{fig:hrg:critical}
\end{figure}


==> pics/hc.tex <==
\scalebox{1.0}{
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 3.5cm/#1,
                  level distance = 0.7cm}] 

\begin{scope}
  \node[node] (root) {}
  child{ node[node] (l) {} 
      child{
          node[node] (ll) {}
           child{
               node[node] (lll) {}
           }
           child{
               node[node] (llr) {}
           }
      }
      child{
              node[node] (lr) {}
           child{
               node[node] (lrl) {}
           }
           child{
               node[node] (lrr) {}
           }
      }
  }
  child{ node[node] (r) {}
        child{
            node[node] (rl) {}
        }
        child{
            node[node] (rr) {}
        }
  };


  \nil{nil}{below of = root, node distance = 3cm}
  \nil{nil2}{below of = root, node distance = 3cm}

  %\nil{nil}{below of = r, node distance = 2.3cm}
  %\nil{nil2}{below of = l, node distance = 2.3cm}

  \pointer{root}{}{e0}{nil2}
  \pointer{lll}{bend right=15}{e0}{nil2}
  \pointer{lll}{bend right=25}{e0}{nil2}
  \pointer{llr}{bend right=15}{e0}{nil2}
  \pointer{llr}{bend right=25}{e0}{nil2}
  \pointer{lrl}{bend left=10}{e0}{nil2}
  \pointer{lrl}{bend right=10}{e0}{nil2}
  \pointer{lrr}{bend left=10}{e0}{nil2}
  \pointer{lrr}{bend right=10}{e0}{nil2}

  \pointer{rl}{bend left=10}{e0}{nil}
  \pointer{rl}{bend right=10}{e0}{nil}
  \pointer{rr}{bend left=10}{e0}{nil}
  \pointer{rr}{bend right=10}{e0}{nil}

  \pointer{r}{bend left}{e0}{root}
  \pointer{l}{bend right}{e0}{root}
  \pointer{rl}{bend right}{e0}{r}
  \pointer{rr}{bend left}{e0}{r}
  \pointer{ll}{bend right}{e0}{l}
  \pointer{lr}{bend left}{e0}{l}
  \pointer{lll}{bend right}{e0}{ll}
  \pointer{llr}{bend left}{e0}{ll}
  \pointer{lrl}{bend right}{e0}{lr}
  \pointer{lrr}{bend left}{e0}{lr}

  \variable{x}{node distance = 1.5cm, right}{root}
  \node[variables] (x2) [node distance=1.5cm, dashed, below of = rr] {$x$}; 
  \path[-, dashed] (x2) edge (rr);
  \variable{y}{node distance = 1.5cm, right}{nil}
\end{scope}


\end{tikzpicture}
}


==> pics/stackabstraction.tex <==
\scalebox{1.0}{
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 3.25cm/#1,
                  level distance = 0.7cm}] 

  \begin{scope}
  \node[node] (root) {2}
  child{ node[node] (l) {} 
      child{
          node[node] (ll) {}
           child{
               node[node] (lll) {}
           }
           child{
               node[node] (llr) {}
           }
      }
      child{
          node[node] {}
           child{
               node[node] (lrl) {}
           }
           child{
               node[node] (lrr) {}
           }
      }
  }
  child{ node[node] (r) {}
  };

  \nilext{nil}{below of = l, node distance = 2.3cm}
  \nilext{nil2}{below of = l, node distance = 2.3cm}
  \nonterminal{B}{below}{r}{B, \Z \Z \Z \,\iBot}
  \tentacle{B}{1}{nil}{-, bend left}
  \tentacleR{B}{2}{r}{-}



  \pointer{lll}{bend left=10}{e0}{nil2}
  \pointer{lll}{bend right=10}{e0}{nil2}
  \pointer{llr}{bend left=10}{e0}{nil2}
  \pointer{llr}{bend right=10}{e0}{nil2}
  \pointer{lrl}{bend left=10}{e0}{nil2}
  \pointer{lrl}{bend right=10}{e0}{nil2}
  \pointer{lrr}{bend left=10}{e0}{nil2}
  \pointer{lrr}{bend right=10}{e0}{nil2}

  \variable{x}{node distance = 1.5cm, right}{root}

  \end{scope}

  \begin{scope}[shift={(4.1,0)}]
      \location{root}{}{2}
      \variable{x}{right}{root}

      \location{left}{below left of = root, node distance=1cm}{}
      \location{right}{below right of = root, node distance = 1cm}{}

      \pointer{root}{}{e0}{left}{}
      \pointer{root}{}{e1}{right}{}
      
      \nilext{nil}{below of = root, node distance=2.3cm}

      \nonterminal{B}{below}{right}{B, \Z \Z \Z \, \iBot}
      \tentacleR{B}{1}{nil}{-, bend left}
      \tentacleR{B}{2}{right}{-}
      
      \nonterminal{Br}{below}{left}{B, \Z \Z \iBot}
      \tentacleL{Br}{1}{nil}{-, bend right}
      \tentacleL{Br}{2}{left}{-}
  \end{scope}

  \begin{scope}[shift={(7.0,0)}]
      \location{root}{}{2}
      \variable{x}{right}{root}

      \location{left}{below left of = root, node distance=1cm}{}
      \location{right}{below right of = root, node distance = 1cm}{}

      \pointer{root}{}{e0}{left}{}
      \pointer{root}{}{e1}{right}{}
      
      \nilext{nil}{below of = root, node distance=2.3cm}

      \nonterminal{B}{below}{right}{B, \Z\,S}
      \tentacleR{B}{1}{nil}{-, bend left}
      \tentacleR{B}{2}{right}{-}
      
      \nonterminal{Br}{below}{left}{B, S}
      \tentacleL{Br}{1}{nil}{-, bend right}
      \tentacleL{Br}{2}{left}{-}
  \end{scope}
\end{tikzpicture}
}


==> preliminaries.tex <==
%The abstraction techniques proposed in this paper rely on several notions of grammars over strings, graphs, and combinations thereof.
Our proposed abstraction techniques rely on several notions of grammars over strings, graphs, and combinations thereof.
We thus briefly recall some basic definitions about context-free grammars alongside with our notation.
%Thus, we briefly recall some basic definitions about context-free grammars alongside with our notation.

%\paragraph{Sets and sequences}
\emph{Sets and sequences.}
Given a set $S$, $\PS{S}$ denotes the powerset of $S$ and $S^{*}$ is the set of all finite sequences (including the empty sequence $\varepsilon$) over $S$.
Moreover, $S^{+} = S^{*} \setminus \{ \varepsilon \}$.
%We usually do not distinguish between a finite sequence $\sigma \in S^{*}$ and the set of all of its elements whenever the meaning is clear from the context.
If $\sigma \in S^{*}$ and $1 \leq k \leq |\sigma|$, where $|\sigma|$ is the length of $\sigma$, the $k$-th element of $\sigma$ is denoted by $\Elem{\sigma}{k}$.
Further, given $\sigma, \tau \in S^{*}$ and $s \in S$, $\Replace{\sigma}{s}{\tau}$ is the syntactic replacement of all occurrences of $s$ in $\sigma$ by $\tau$.

%\paragraph{Partial functions}
\emph{Partial functions.}
Given a partial function $f : S \to D$, we write $f(s) = \pBot$ if $f$ is undefined on $s$.
The restriction of $f$ to domain $T \subseteq S$ is $\Proj{f}{T}$.
Further, the sequential composition of partial functions $f : S \to T$, $g : T \to R$ is denoted by $f \FComp g$, i.e. $(f \FComp g)(s) = g(f(s))$.
%We often tacitly lift functions to functions on sets and sequences by pointwise application.
For a partial order $(D,\sqsubseteq)$, $f \,\dot{\sqsubseteq}\, g$ denotes that functions $f, g : S \to D$ are ordered by pointwise application of $\sqsubseteq$.

%\paragraph{Binary relations}
\emph{Binary relations.}
Given a binary relation, say $\Rightarrow\;\subseteq S \times S$, we denote the \emph{inverse} of $\Rightarrow$ by $\Leftarrow$.
That is, $s \Leftarrow t$ iff $t \Rightarrow s$.
Moreover, $s \nRightarrow$ denotes that there exists no element $t \in S$ such that $s \Rightarrow t$.
The reflexive and transitive closure of $\Rightarrow$ is $\Rightarrow^{*}$.
Analogously to functions, $R_1 \FComp R_2$ denotes the composition of binary relations $R_1$ and $R_2$, i.e. $R_1 \FComp R_2 = \{ (u,w) ~|~ \exists v : (u,v) \in R_1, (v,w) \in R_2 \}$.

%\paragraph{Context-free string grammars}
\emph{Context-free string grammars.}
Let $I_N$ and $I_T$ be disjoint finite sets of \emph{nonterminal} and \emph{terminal} symbols.
A \emph{context-free string grammar} (CFG) over $I = I_N \cup I_T$ is a finite set
$\iC \subseteq I_N \times I^{+}$ of rules of the form $X \to \sigma$.\footnote{We only consider sets of non-empty strings and thus exclude the empty string $\varepsilon$.} 
Given two sequences $\sigma,\tau \in I^{+}$, we say that $\iC$ \emph{directly derives} $\tau$ from $\sigma$, written $\sigma \iDerive{\iC} \tau$, if there exists a rule $(\Rule{X}{\rho}) \in \iC$, $\sigma = \sigma_1 X \sigma_2$, and $\tau = \sigma_1 \rho \sigma_2$.
%An \emph{inverse derivation} $s \rDerive{C} t$ is defined as $t \iDerive{C} s$.
%Moreover, $\iDerive{C}^{*}$ and $\rDerive{C}^{*}$ denotes the reflexive and transitive closure of $\iDerive{C}$ and $\rDerive{C}$, respectively.
The \emph{language} of a CFG $\iC$ is given by the function $\iL{\iC} : I^{+} \to \PS{I_T^{+}}$ with
%$\iL{\iC}(\sigma) = \{ \tau ~|~ \sigma \iDerive{\iC}^{*} \tau ~\text{and}~ \tau \in I_T^{*} \}$.
$\iL{\iC}(\sigma) = \{ \tau \in I_T^{+} ~|~ \sigma \iDerive{\iC}^{*} \tau \}$.
%
Similarly, the \emph{inverse language} of $\iC$ is given by the function $\rL{\iC} : I^{+} \to \PS{I^{+}}$ that takes a string and applies inverse derivations to it as long as possible.
That is,
$\rL{\iC}(\sigma) = \{ \tau \in I^{+} ~|~ \sigma \rDerive{\iC}^{*} \tau ~\text{and}~ \tau \nrDerive{\iC} \}$. %, where $t \nrDerive{C}$ denotes that no inverse derivation is applicable to $t$.
%
%An important class of CFGs %that will be employed to refine abstraction and concretization 
%are \emph{right-linear grammars}, i.e. for every rule $\Rule{X}{s}$, $s \in T^{+}$ or $s \in T^{+}N$.
%Finally, a CFG $C$ is called \emph{backward confluent} if its inverse language is a singleton for every possible string, i.e. $\forall s \in I^{*} : |\iLang{C}{s}| = 1$.


